An Adaptive Benchmark for Modeling User Exploration of Large Datasets

In this paper, we present a new DBMS performance benchmark that can simulate user exploration with any specified dashboard design made of standard visualization and interaction components. The distinguishing feature of our SImulation-BAsed (or SIMBA) benchmark is its ability to model user analysis goals as a set of SQL queries to be generated through a valid sequence of user interactions, as well as measure the completion of analysis goals by testing for equivalence between the user's previous queries and their goal queries. In this way, the SIMBA benchmark can simulate how an analyst opportunistically searches for interesting insights at the beginning of an exploration session and eventually hones in on specific goals towards the end. To demonstrate the versatility of the SIMBA benchmark, we use it to test the performance of four DBMSs with six different dashboard specifications and compare our results with IDEBench. Our results show how goal-driven simulation can reveal gaps in DBMS performance missed by existing benchmarking methods and across a range of data exploration scenarios.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> contents/4_spec_old.tex <==
%-------------------------------------------------------------------------------
\section{Specifying Allowable Actions}
\label{sec:allowable-actions}


\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/layers_update2.pdf}
    \caption{(A) Shows how relationships between dashboard components are captured in the SIMBA graph layer. Here, the checkbox widget of the Customer Service Dashboard can trigger updates in the main visualizations in green and summary statistics in blue. These updates trigger new SQL queries in the data layer to be executed by the DBMS, shown in (B) and (C). Finally, (D) shows all of the relationships in the graph layer for the customer service dashboard.}
    \label{fig:layers_update}
\end{figure*}


Given a specified user goal, the next step is to detect which actions bring a user towards their goal. Currently, we can express goals in the form of query templates, but we lack consistent data structures for inferring what interactions a user is allowed to perform in a given dashboard, and how these interactions may translate to queries on an underlying dataset. To address this problem, we propose a specification language, which allows dashboard developers to \emph{specify any dashboard design} consisting of common visualization and interaction components.
Our specification language borrows elements from IDEBench \cite{idebench} and is inspired by existing visualization tools such as Polaris/Tableau~\cite{stolte2002polaris}, Vega-Lite~\cite{2017-vega-lite}.

What is novel about our approach is not the language itself, but how we use it to generate a \emph{graph layer} of the desired dashboard. \joanna{We should discuss novelty of this one more time to make sure that what we're claiming doesn't overlap with IDEBench or VegaLite.} 
\leilani{Agreed. Honestly, I wonder if we really even need to claim any novelty here. I would argue not. In which case, we can save a lot of space by just saying we build on prior work and cutting out the details.}
With this graph data structure, we can infer relationships between the visualizations in the dashboard, the interaction widgets an analyst might use to manipulate these visualizations, and their corresponding SQL queries.
%Our graph representation also allows us to translate any visualization or user interaction to its corresponding SQL queries, so we can reason about how these visualizations and interactions operate within the underlying data space.
In other words, we can reason about any possible interaction a user might perform on this dashboard by maintaining a \emph{joint representation} of the dashboard state:
\begin{itemize}
\item \textbf{interaction layer}: tracks dashboard state as positions within and updates to the graph representation; and
\item \textbf{data layer}: translates the user's graph manipulations to their corresponding SQL queries on a back-end DBMS.
\end{itemize}
In this section, we briefly summarize our specification language, explain how we translate dashboard specifications into our graph representation, and discuss how we map user interactions (i.e., manipulations on the graph) to their corresponding SQL queries.

%\leilani{This section should motivate why specification languages are important for dashboard development. The related work should probably provide a brief overview of available languages before we get here.}
%In order to capture interactivity usage and change over time, we develop a specification language inspired by Vega Lite \cite{2017-vega-lite} to express the capabilities of a visual interface and interaction sequences. A specification standard allows us to benchmark dashboards written in all languages, but not yet including all possible visualizations.



\subsection{Specification Language}
\label{sec:allowable-actions:spec-language}
% \joanna{
% \begin{itemize}
%     \item introduce specification language to capture dashboard capabilities and history of interactions
% \end{itemize}
% }
% \leilani{remove refs to non-customer service dashboards.}
% Our specification language enables a benchmark user to specify a desired dashboard design that queries a target dataset file.
% It merges language structure from Vega-Lite~\cite{2017-vega-lite} (for UI specification) and IDEBench~\cite{idebench} (for query specification).
% Our specification language is not necessarily a novel contribution in itself. However, to understand the SIMBA benchmark, the reader needs to know how this language works. Hence we provide a brief summary here.
% %Dashboards and their associated user exploration sessions are represented via three specification documents.
% Our specification has three parts: a \emph{database specification} to describe the input dataset, an \emph{interface specification} to describe the visualizations and interactions in the dashboard, and finally an (optional) \emph{interaction specification} that allows the benchmark to replay an existing file containing pre-recorded system interaction logs.
% %The dataset that the dashboard is built upon is represented in a \emph{database specification}. An \emph{interface specification} defines visualizations and interactive elements as connections between the fields expressed in the dataset specification. Finally, the \emph{interaction specification} captures real or synthetic \emph{exploration sessions} that are expressed within the context of the dashboard specification. An exploration session is a sequence of interactions a user performs to accomplish a data exploration goal with a given dashboard.

% %Our specification structure builds directly on existing languages, including the specification interface to IDEBench~\cite{idebench} and relevant visualization specification languages like Vega-Lite~\cite{2017-vega-lite}. We describe our specification language not necessarily as a novel contribution in itself, but to inform downstream components of the benchmark and it's functionality.
% %: how we generate graph representations of dashboards, how we translate interactions to SQL queries, and how we use the graph representations to simulate realistic interaction sequences.



% \subsubsection{Database Specification}
% The database specification is a JSON representation of the datasets that support the visualizations, similar to prior work~\cite{idebench}. Each table is specified in a de-normalized, star schema form using key-value pairs for each column name and datatype (categorical, numerical, datetime).
% However, unlike previous benchmarks, the SIMBA benchmark also supports the specification of calculated fields, which are common in dashboard development.
% Calculated fields are specified using key-value pairs, with the key being the alias for the calculated field and the value being the SQL query performing the calculation.
% %Any custom calculated fields that are utilized to produce a visualization in the dashboard are also defined within the database specification, expressed as column name-SQL pairs.
% %Dashboard visualizations may only be constructed from the fields present in the specification, but combinations of table columns, basic aggregations over numerical table columns, and custom fields are all supported.

% %Due to its high-level format, our database specification is easily defined and portable across a variety of DBMSs. In the following sections, we demonstrate our benchmark over a set of common DBMSs tested in prior work (SQLite, PostgreSQL, DuckDB, MonetDB)~\cite{idebench, crossfilter}.
% %%using drivers derived from previous interactive data exploration benchmarks \cite{idebench, crossfilter}.

% \subsubsection{Interface Specification}
% The interface specification essentially extends Vega-Lite to make it easier to specify complete dashboards rather than just a single visualization. It captures three sets of components: \emph{visualizations} (e.g., tables, bar charts, line charts, etc.), \emph{widgets} (check boxes, sliders, dropdown menus, etc.), and \emph{relationships} between the two (see \autoref{fig:layers_update} for examples).
% %The visual components of a dashboard are broken into \textit{visualizations}, such as tables, graphs and maps and interaction based \textit{widgets}, elements of a dashboard that are used to manipulate visualizations. Example widgets include sliders, dropdown menus, checkboxes, and even the visualizations themselves, such as in the case of brushing and linking.
% Note that visualizations themselves can also be interactive widgets, such as in brushing and linking.~\cite{crossfilter}. 
% Relationships map dependencies between widgets and visualizations into queries,
% %Relationships capture source-target relationships between visualizations and widgets, as well as which data attributes are manipulated,
% for example how a slider widget modifies or extends corresponding SQL filter predicates.
% %The graph layer in Fig~\ref{fig:layers_update} demonstrates a visual decomposition of the Customer Service dashboard into visualizations, widgets and the relationships between them.

% The SIMBA benchmark can also simulate \emph{manipulation} of the interface itself, for example to swap out an attribute on the x- or y- axis of a visualization or even to add/remove entire visualizations. These capabilities are expressed through \emph{wildcards}, which are placeholders that tell the benchmark
% %to explore all possible options at a particular position in the graph %representation. For example, inserting a wildcard within a specified visualization tells the SIMBA benchmark
% which visualization parameters are permutable, e.g., that the x- and y-axes could be changed through interface manipulations. We discuss this further in \autoref{sec:allowable-actions:graph-layer}.

% %However, visualizations and widgets only specify which components appear in the dashboard and not the relationships that govern their behavior, such as which visualizations are affected by a slider widget, or which visualizations are affected when a user brushes a histogram in a crossfilter dashboard~\cite{crossfilter}.
% %The interactivity within and across visualizations and widgets is captured as directed \textit{relationships}. Relationships are used to express cases where a source widget filters one or more target visualizations, such as the queue checkbox that filters all three visualizations in the Customer Service dashboard in \autoref{fig:customer_service}.
% %%They can also express direct interactions between $n$ visualizations such as brushing and linking.
% %Relationships capture source-target relationships between visualizations and widgets, as well as which data attributes are manipulated, for example how a filter predicate may be modified in or added to the corresponding SQL query. The graph layer in Fig~\ref{fig:layers_update} demonstrates a visual decomposition of the Customer Service dashboard into visualizations, widgets and the relationships between them.
% %%Each relationship is defined over a set of data attributes, allowing for fine-grained specification of interaction.
% %%\joanna{Wildcards}


%  %\begin{figure}[t]
%  %   \centering
%  %   \includegraphics[width=\columnwidth]{figures/database_example.png}
%  %    \caption{An example of a table represented in the database specification. In this case %there is a single table named "covid" with two categorical attributes and two numerical attributes.}
% %     \label{fig:db_spec}
% % \end{figure}


% \subsubsection{(Optional) Interaction Specification}

% The interaction specification is an array of timestamped interaction logs defined with respect to the interface specification, based on the IDEBench logging structure~\cite{idebench}. Each log record
% %represents a manipulation of a specified relationship.
% %Each item in the interaction specification is
% represents either a \textbf{data manipulation} executing a relationship defined in the interface specification, or an \textbf{interface manipulation} redefining a piece of the interface specification.
% %expressed as instantiations of one of the relationships defined in the interface specification.
% Each interaction log record must contain a timestamp, the triggered relationship and the new values for the data attributes activated by the specified interaction, i.e., the query results. When many relationships are defined, a single interaction might trigger a chain of updates across the dashboard. However, only the relationships directly triggered by the logged interaction, i.e., the first interaction within a chain, are defined as ``user'' interactions. Subsequent dashboard updates, i.e., the rest of the chain, are propagated automatically by the benchmark using the interface specification and are assumed to occur simultaneously.

%The interaction specification can be used to map existing system interaction logs into the SIMBA benchmark's target format to test against ground truth, as well as to generate the synthetic workloads described in \autoref{sec:simulation}.
%Workloads generated from user sessions can be directly specified using the interaction specification format or generated synthetically as described in Section~\ref{sec:simulation}.
%%Interface manipulations are only possible when one or more wildcards exist in the interface specification. As an interaction session unfolds, each time a new value is selected for the wildcard, a working version of the specification is updated to reflect the change.

\leilani{It seems we can save a lot of space here by just saying we merge the specifications of IDEBench and Vega-Lite to provide more expressive inputs to our benchmark. Like IDEBench, we have an interface specification and a database specification. However, IDEBench provides limited support for expressing interactions. Thus, we merge it with an abbreviated version of the Vega-Lite language to enable benchmark users to specify interactions and how they impact different dashboard components within the interface specification. That being said, our language format is largely the same as existing languages, so we do not cover it in detail here.}

\leilani{Joanna, can you do another pass to basically comment out all this other stuff in 
 Section 3.1 and replace it with a paragraph similar to what I described?}

Our specification language enables a benchmark user to specify a desired dashboard design that queries a target dataset file.
It merges language structure from Vega-Lite~\cite{2017-vega-lite} (for UI specification) and IDEBench~\cite{idebench} (for query specification).
Our specification language is not necessarily a novel contribution in itself, but to understand the SIMBA benchmark, the reader needs to know how this language works. Hence we provide a brief summary here. This language is divided into three essential components: the Database Specification, Interface Specification, and an optional Interaction Specification. 
    % Each plays a pivotal role in ensuring the dashboard not only displays data effectively but also facilitates an engaging user experience conducive to exploring and understanding customer service metrics. 
    % We will use our earlier example of the Customer Service dashboard to illustrate a dashboard is represented in this framework.

\subsubsection{Database Specification}
The database specification is a JSON representation of the datasets that support the visualizations, adapted from IDEBench ~\cite{idebench} to allow for the declaration of parameters and custom fields. 
% At the heart of a successful customer service dashboard is its database, the primary source of data for analysis and visualization. The Database Specification details how this data is structured and prepared for dashboard use. 
It employs a JSON format with a star schema design, which clearly outlines each column’s name and type (e.g., categorical, numerical, datetime) and includes provisions for calculated fields. The specification may be ported across DBMSs, but care must be taken to author calculated fields in a SQL dialect agnostic manner.
% This meticulous approach to data organization ensures that the dashboard can leverage diverse data sources effectively, laying a solid foundation for insightful customer service analytics.

\subsubsection{Interface Specification
}
The interface specification essentially extends Vega-Lite to makes it easier to specify complete dashboards rather than just a single visualization. Beyond mere data representation, the Interface Specification focuses on the dashboard's user interaction and presentation layer. It leverages the principles of Vega-Lite to simplify the creation of comprehensive and interactive dashboards. This specification includes a range of visualization options (charts, tables, etc.) and interactive elements (sliders, dropdowns) to enhance data exploration. It defines how these elements interconnect, such as how a slider adjustment might refine the data displayed in a chart, facilitating an intuitive and dynamic user experience (see \autoref{fig:layers_update} for examples). The emphasis here is on creating dashboards that are not just visually attractive but are truly interactive platforms for users to engage with and derive meaningful insights from customer service data.

\subsubsection{Interaction Specification }
The interaction specification is an array of timestamped interaction logs defined with respect to the interface specification, based on the IDEBench logging structure~\cite{idebench}. Each log record
represents either a \textbf{data manipulation} executing a relationship defined in the interface specification, or an \textbf{interface manipulation} redefining a piece of the interface specification. While the first two specifications address the dashboard's structure and presentation, the Interaction Specification introduces a dynamic element by documenting user interactions with the dashboard. The Interaction Specification may take the form of logs collected from an observed user session or can be generated for a theoretical dashboard as explained in Section \ref{sec:simulation}.
% This feature captures each interaction in a timestamped log, including data manipulations and interface adjustments. Such detailed recording is crucial for several reasons: it enables the replay and review of customer service sessions for enhanced understanding of dashboard engagement patterns and identifies areas for improvement. This insight is invaluable for iterative dashboard development, ensuring it remains aligned with customer service needs and preferences.


\subsection{Generating the Interaction Layer}
\label{sec:allowable-actions:graph-layer}

\leilani{I wonder if we can also save space by cutting this subsection entirely. We can assess later once the new Section 4 is in the paper.}

The interaction layer is a graphical representation of the Interface Specification. We first initialize each interactive dashboard element in the specification and then draw a directed edge from a source element to a target element if interaction with the source element precipitates a change in the target element. For example, in the case of a filtering dropdown element, an edge would be drawn from the dropdown to the visualization that it filters. Within each node of the graph we save properties such as the fields used in the visual element and any filters that are currently applied.
    To simulate a user interacting with the dashboard, we play the interactions in the Interaction Specification across the graph. As we do so, we encounter two types of interactions: \emph{data manipulations}, which broadly refer to filtering actions, and \emph{interface manipulations} which capture a change to the dashboard definition.

\subsubsection{Initial Graph Generation for Customer Service Dashboard}We initialize the initial graph with six nodes, one checkbox and five visualizations, with their composite fields as node properties. Next, we note in \autoref{fig:layers_update} that the checkbox filters every visualization in the dashboard. Therefore, we draw five directed edges originating from the checkbox node and targeting each visualization. We continue drawing edges until we exhaust the interactions listed in the Interface Specification.

\paragraph{Graph Updates From Data Manipulations} Simulating a user interaction with a widget (e.g., moving a slider, checking a check box) induces a \emph{data manipulation} in the graph layer. For instance, a customer service representative selecting queue \textbf{A} in the checkbox will filter all five visualizations in the dashboard. In this case we first locate the source element of the interaction, the checkbox node, and update the node properties to reflect that it has been filtered down to queue A. Next, we propagate this filter across all outbound edges of the checkbox node. For each target node connected by an edge, we add the filter condition to the list of node properties. We then check each target nodes for outbound edges and once again propagate the filter condition if any exist. These two steps repeat until either all nodes have the filter condition applied or there are no longer any outbound edges to traverse.

\paragraph{Graph Updates From Interface Manipulations}
Previous benchmarks either place no restrictions on the dashboard design space  \cite{idebench} focus exclusively on bar charts (e.g., IDEBench~\cite{idebench}) or assume that dashboard structure is immutable (e.g., Crossfilter~\cite{crossfilter}). Unlike these benchmarks, our approach embraces the dynamic nature of dashboards, allowing visual elements of any type to be edited and for interactions to be redefined through the use of wildcards. Wildcards allow for the adaptation of the dashboard design, enabling actions such as adding a new metric visualization based on recent customer service inquiries or adjusting existing visualizations to highlight trends in customer satisfaction.
    The Customer Service Dashboard does not support interface manipulations, but we can imagine a case where the author goes back and edits the dashboard to add a dropdown filter for RepresentativeID. The author would create the new visual element and then define filter relationships between it and the rest of the elements of the dashboard. Each of these actions results in an interface manipulation.
     When an interface manipulation is triggered, we first check that the manipulation is valid as per the interface specification. Then, we insert the new visual element or interaction into the Interface Specification and initialize the graph layer anew.

% % If the interface specification contains wildcards, then interface manipulations could alter the interface graph. For example, wildcards might add/alter an encoding in a visualization (e.g., add a color scale, change the x- or y-axis, etc.) or remove a visualization from the interface.
% \revised{For example, in response to a series of customer interactions highlighting a new service issue, a wildcard might be used to introduce a new visualization that tracks this issue over time. This flexibility allows customer service dashboards to remain relevant and informative as the service landscape changes.
% }


\subsection{From Interactions to SQL Queries}
\label{sec:allowable-actions:interactions-to-sql}

\leilani{I thought the updated version of Section 3 was supposed to explain that (1) just because you write a goal doesn't mean that goal is meaningful for a given dashboard, so (2) we need a way of assessing whether a given goal makes sense for a given dashboard. I don't see anything like that in the latest version of Section 3.}

\leilani{I like having a walkthrough of the different specification layers. We can keep this subsection 3.3 for now, but we should trim/remove the prior subsections IMO and add content about how we go from a general goal using our algebra to a specific goal for a given dashboard.}

The SIMBA benchmark uses the graph layer to facilitate bi-directional mapping between interaction records (interaction layer) and SQL queries (data layer), as demonstrated in \autoref{fig:layers_update} and \autoref{sec:allowable-actions:graph-layer} for the Customer Service dashboard. For each data manipulation, filter statements are propagated across the dashboard graph for each node that can be reached via directed edges. The additional filter statements alter the data that should be displayed in each visual element. Therefore, we need to craft a query to fetch the modified data from the DBMS using the data layer.

The data layer represents each node as SQL query where the node properties in combination with the Database Specification define how the SQL query is crafted. In the case of a data manipulation, we can compile each node and obtain the set of SQL queries that would be executed against the DBMS when the interaction occurred. Returning to the example from \autoref{sec:allowable-actions:graph-layer}, at the conclusion of the 'Select Queue' checkbox action there are five visualization nodes with property updates. For each of these nodes,  a new SQL query to be generated in the data layer.

In the Customer Service dashboard example, when the interaction layer was initialized a node was created for each visual element and each node was sent to the data layer. The set of fields used in each visualization were cross-checked against the Database Specification to identify their parent table or custom field definition. The validated fields are added to the SELECT statement and their parent tables are joined according to the Database Specification and added to the FROM statement. By this process, the SQL query for the Lost Calls visualization would look like SELECT COUNT(lostCalls) FROM customerService;

Continuing the example in  \autoref{fig:layers_update}, when the checkbox widget updated the \textbf{queue} selection to \textbf{A}, each traversed node in the interaction layer was updated to \textbf{A}. Therefore, we update the \textit{WHERE} clause in each query to include a phrase "AND queue = 'A' ". These queries are then recorded in the workflow attached to the trigger interaction.

==> contents/5_seq.tex <==



\subsection{Simulating Targeted Exploration}
\label{sec:simulation:targeted}
% \leilani{fill in, stuff about generating sequences to achieve a specific goal}
% write up a definition for exploration end states/goal states using Tableau NLP studies, viz rec and crossfilter
Targeted exploration describes cases in which the user has a well-formed analysis goal in mind.
%For example, a call center manager might want to use the Customer Service dashboard to determine which call center representatives are the highest performers, as determined by the number of calls they respond to. In addition to determining which reps had the most calls overall, the manager might look at the overall calls per hour to see if someone was a high performer on a particular shift or if there are outlier performers that might need further investigation.
%
%\subsubsection{Overview: The Structure of a Simulation}
% \leilani{summarize where the simulation starts, how each individual step/interaction is generated, and how progress is measured. should be very brief, just intro to the other subsubsections.}
%Targeted exploration is simulated with a set of parameterized goal templates (see \autoref{sec:goals:templates} for details).
%where each template represents a related analysis question within a central theme, such as, \emph{``Which reps are high performers?''} These templates are translated into a dashboard simulation that outputs a workflow of queries that can be executed against a DBMS.
%
To execute a targeted simulation, the SIMBA benchmark requires a dashboard specification (as stipulated in \autoref{sec:allowable-actions:spec-language}) and a set of goal templates to be achieved (as stipulated in \autoref{sec:goals:templates}).
%To execute a targeted simulation, users need a set of templates (expressed as the interaction specification and associated configuration) and specifications for the dataset and dashboard. First, 
The specification is used to construct a graph representation of the dashboard.
%the dashboard is initialized as a graph from the set of specification documents.
Then, a goal template is selected from the input set and decomposed into its corresponding goal queries. Next, the graph is searched to identify a set of dashboard states that achieves all of the goal queries, with preference given to states that achieve more than one goal simultaneously. Then, the sequence of interactions needed to achieve each desired goal state are recorded as well as the corresponding SQL queries, which are inferred from the graph representation. These interactions and queries comprise the benchmark workflow.
%, and as they are executed against the graph, the queries generated from each step form the query workflow.

Simulations are executed recursively on the dashboard graph and array of goal templates until either no goal templates remain or a single template is deemed unsolvable.
More complex workloads can also be composed by forming ordered lists of goal query sets. We present three example compositions from the literature in \autoref{sec:evaluation}.
%Given an array of goal templates to achieve in sequence, simulations are executed recursively on the dashboard graph until either no goal templates remain or a single template is deemed unsolvable.
%Once a template is solved, we proceed to the next template in the sequence. Otherwise, a search across the dashboard graph is initiated to determine the next user interaction.

\subsubsection{Generating Immediate Next Steps}
% \leilani{about generating the current available interactions given the current dashboard state.}
Given the current state of the dashboard, the simulator must decide the next step to accomplish the current goal template. The simulator leverages the joint representation by searching over manipulations in the graph layer, and checking the SQL layer to determine if analysis goals have been met. For example, in \autoref{fig:goal_to_queries} an Analyzing Spread template is executed against the Customer Service dashboard. To generate the next interaction step, we search the graph layer to find all possible manipulations, then test to see which steps achieve at least one of the four goal queries using the SQL layer. We then choose a step that maximizes the goal queries achieved and the goal queries that would be achieved with one additional graph interaction.

% Given these possible future interaction states, we developed
% an Oracle model that estimates the shortest path from the current dashboard state to the target goal state, and selects the next state that brings the simulation closest to the goal state.



\subsubsection{Measuring Goal Completion}
\label{sec:simulation:goal-completion}

A key challenge in generating goal-directed simulations is measuring progress towards the specified goal. How does the simulator know when the goal has been achieved? To measure progress towards a given goal, i.e., a populated goal template from \autoref{sec:goals}, we track the SQL queries generated by the dashboard with each simulated interaction, and compare the simulated SQL queries with the specified goal queries.
%A specified goal query is considered solved if the result set produced by the queries representing the current dashboard configuration includes the result set generated by the template \joanna{There's a more mathematical (set theory) way to phrase this.}.

\paragraph{Determining Goal Completion.} At a high level, we consider a target goal query solved if the result set of this query is ``covered'' by the result sets of all simulated SQL queries thus far. In other words, if at some point in the simulation the user saw the desired records specified by the goal query, then this goal has been achieved.
This is essentially a comparison of two sets. The first set represents the anticipated query results from the specified goal query, which we denote as $R_g$. If there are two goals to achieve $g$ and $g'$, we can represent this as a union of the result sets across the corresponding goal queries: $R_g \cup R_{g'}$, which also extends easily beyond two goals. The second set is the set of observed query results for each simulated interaction thus far. For example, if only one interaction has been simulated $i$, then there is only one result set to compare, denoted as $R_i$. If two interactions have been simulated $i$ and $i'$, we denote this as $R_i \cup R_{i'}$. Given the set of all goals $G$ and the set of all simulated interactions $I$, we consider all target goal queries solved if:
\begin{equation*}
    \bigcup_{g \in G} R_g \subseteq \bigcup_{i \in I} R_i
\end{equation*}
%Given a simulated query and a target goal query, the goal query is considered solved if the result set produced by the simulated query \emph{subsumes} the result set of the goal query.

We can determine the equivalence of query result sets in three ways: (1) \emph{syntactical equivalence}, or seeing if the text of the queries is the same, (2) \emph{semantic equivalence}, or reasoning about what the queries represent to see if the results should be the same, or (3) \emph{result equivalence}, or executing the queries and inspecting the results to test if they overlap. We can use similar techniques to test for query subsumption, for example if one query is the prefix of another query in terms of text, or if semantically one query should subsume the other. We describe our equivalence/subsumption methods below.

\paragraph{Syntactical Equivalence.} A query is syntactically equivalent to the goal query if the query's text covers at least the same columns and rows as the goal query's text. Consider the following example:
\begin{example}
\emph{Revisiting the target goal query in Example~\ref{ex:example-question}, we consider the following query to subsume this goal query, since it is syntactically the same minus an added group by attribute (\texttt{queue}):}
\vspace{-1mm}
\begin{verbatim}
SELECT hour, queue, COUNT(*) as call_volume,
    sum(abandoned) as call_abandonment
FROM customer_service GROUP BY hour, queue
\end{verbatim}
\vspace{-1mm}
\emph{To get equivalent results to our original goal query (i.e., only group by hour), we aggregate the results further to remove the \texttt{queue} attribute.}
\end{example}
%the query result set subsumes the result set of the goal query. Specifically, all of the columns and rows present in the goal query result set are likewise present in the query result set.

%The semantics of SQL queries is formally defined by stating a set of rules that determine a syntax-driven translation of an SQL query to a formal model. Methods for equivalence testing include comparing overlap in result sets \cite{}, and parsing SQL queries to find similarities in the statement's syntactical structure \cite{}. We leverage a combination of both methods to determine when a goal template has been achieved.

\paragraph{Semantic Equivalence.} We use the SPES SQL solver~\cite{zhou2020spes} to infer semantic equivalence between goal queries and dashboard interaction queries. %SPES is a SQL solver for inferring semantic equivalence between SQL queries~\cite{zhou2020spes}.
Two queries are equivalent if they produce the same results given any valid input relations, which SPES infers by compiling SQL queries into denotational semantics and using mathematical principles to reason about them.
%We use SPES to check the equivalences of our true goal queries with the corresponding dashboard goal queries, and found that although it is able to perform well, 
However, there are some SQL features that SPES does not support such as expressions in \verb|GROUP BY| clauses, aggregate functions such as \verb|MAX()| and \verb|MIN()|, and functions that extract values from existing data such as \verb|YEAR()| and \verb|MONTH()| from a date. For this reason, we augment SPES with two additional methods for equivalence testing: result set overlap and string matching.
For example, we infer equivalence if SPES returns a match or if string matching indicates >95\% similarity after processing to remove additional whitespace.
 
 \paragraph{Result Equivalence.} Query results are considered equal when the goal query result is subsumed by the query results represented in the current dashboard state. Specifically, every column and row in the goal result set must also be present in the dashboard result set, but the dashboard may contain more rows or columns than what is stipulated in the goal query.
 %Each visualization in the dashboard is represented by a single query that is at the same level of aggregation as the visualization. 
 For example, if the goal result is a subset of the query results rendered in a specific visualization component, then result equivalence can be detected in the dashboard.
 %Therefore, to achieve result equivalence it is sufficient that the goal result is a subset of the test result-- that the required data is present in the visualization, although additional information might be present.
 
 \paragraph{Measuring Progress.} Given the ability to determine SQL equivalence or subsumption, goal completion becomes straightforward to detect. However, making progress towards a goal is not the same as completing it. We measure progress toward a specified goal as \emph{overlap} between result sets rather than subsumption or equivalence. The more results are ``covered'' by a potential interaction (i.e., the more results overlap with the anticipated result set), the closer it brings the simulation to reaching the target goal state. In this way, the Oracle model can compare the utility of potential next steps by comparing overlaps produced by their corresponding query result sets (i.e., maximizing $\bigcup_{g \in G} R_g~~~\bigcap~~~\bigcup_{i \in I} R_i$).

==> contents/7_discussion.tex <==
\section{Limitations and Future Work}
\label{sec:discussion}

